Bi-SIS Epidemics on Graphs -- Quantitative Analysis of Coexistence Equilibria

We consider a system in which two viruses of the Susceptible-Infected-Susceptible (SIS) type compete over general, overlaid graphs. While such systems have been the focus of many recent works, they have mostly been studied in the sense of convergence analysis, with no existing results quantifying the non-trivial coexistence equilibria (CE) - that is, when both competing viruses maintain long term presence over the network. In this paper, we prove monotonicity of the CE with respect to effective infection rates of the two viruses, and provide the first quantitative analysis of such equilibria in the form of upper bounds involving spectral radii of the underlying graphs, as well as positive equilibria of related single-virus systems. Our results provide deeper insight into how the long term infection probabilities are affected by system parameters, which we further highlight via numerical results.

==> Sections/outline.tex <==

Section 1:

Towards then end: one paragraph on basic notation


Section 2: Primer on SIS model

-> Introduce single SIS
    -> Talk about main result and some history (can also show convergence results using MDS)
    -> Give the survival condition $rho_A > 1$
    -> Use this section to set up notations such as x*, y*

    
-> Introduce bi-SIS
    -> Previously we had two types equilibrium. Now there are 3 types.
    -> Under certain condition (CE condition) both viruses survive, while otherwise system eventually boils down to single virus system (WTA).
    -> MDS is also one of the key properties, and our previous work showed convergence.
    -> Informally form analogy $rho*_A > 1$ and $rho*_B > 1$ is the survival condition, in addition to $rho_A>1$ and $rho_B>1$
    -> Later on we will explain this in more detail with the help of an illustration/figure
    -> (Option either here or only in section 4) mention that there can be multiple, disjoint CE fixed points.
    -> Point out to our paper for the most recent results.
    
-> Emphasize once again that there is no result yet to quantify the CE fixed point


Section 3:

In general: We do not claim that we are the first ones ever to give quantitative results. However, we add to existing results by meighem by providing useful bounds on avg X. Avg X is what usually matters instead of individual entries (many ways to explain this: large graph, etc. Cannot know degree of each node in detail, etc etc.)


Building up on the discussion in section 2, we first provide quantitative bounds on the positive equilibrium under survival condition.

-----
Theorem:

-----

Talk about special case: regular graph. Everything coincides. Can reproduce known result from Meighem's paper.

Talk a bit about use case: Gives bounds directly on avg X instead of Xi - particularly useful for cases such as large graph etc.


Section 4:

Again sort of building up on discussion in section 2: First we mention that MDS property is useful since it helps us get started with the following:

Lemma: We have $\partial y_i/\partial \tau_1 <= 0$ and $\partial x_i/ \partial tau_1 >=0$
(proof will rely on citing the previous paper for MDS results)

This key property helps us build the following results:

Proposition: fi = y/1-x is decreasing in tau1, etc.....
(proof will be slightly long)

Give interpretation of the proposition. A few lines for conditional probability explanation, etc. Basically saying that this is not just one decreases and other increases, it is sharper.

Proposition: y < y*(1-x) and x < x*(1-y)


The proposition has the following corollary, which helps us establish bounds on avgX + avgY

Corollary: avgX + avgY <= 1 - 1/(rhoA + rhoB  - 1)

1) Explain interpretation when rhoA and rhoB are close to 1 (and as a result even rhoA* and rhoB* are close to 1). Then, avgX + avgY is also very small.
2) Draw the figure and explain this
3) When either one of the two is close to 1, it is almost the same as single virus bound - so there is consistency with previous result.
4) when either of the two are less than 1, then just use single virus bound as is instead of this bound.

